A Generalized Minimax Q-learning Algorithm for Two-Player Zero-Sum Stochastic Games

We consider the problem of two-player zero-sum games. This problem is formulated as a min-max Markov game in the literature. The solution of this game, which is the min-max payoff, starting from a given state is called the min-max value of the state. In this work, we compute the solution of the two-player zero-sum game utilizing the technique of successive relaxation that has been successfully applied in the literature to compute a faster value iteration algorithm in the context of Markov Decision Processes. We extend the concept of successive relaxation to the setting of two-player zero-sum games. We show that, under a special structure on the game, this technique facilitates faster computation of the min-max value of the states. We then derive a generalized minimax Q-learning algorithm that computes the optimal policy when the model information is not known. Finally, we prove the convergence of the proposed generalized minimax Q-learning algorithm utilizing stochastic approximation techniques, under an assumption on the boundedness of iterates. Through experiments, we demonstrate the effectiveness of our proposed algorithm.

==> Implementation.tex <==
\section{Model-free Generalised Minimax Q-learning} \label{impalg}
\color{black}
Note that an input to the Algorithm \ref{alg:minimax Q-learning} is the relaxation parameter $w \leq w^*$, where $w^*$ is defined in \eqref{w-star}. As $w^*$ depends on the transition probability matrix $p$, it is not possible to directly use it in the experiments, where we do not have access to the model. In this section, we describe our model-free generalised minimax Q-learning procedure where the parameter $w$ is updated iteratively from the samples. 

We maintain a count matrix $C_n[i][j][u][v], ~ \forall i,j \in S, u \in U, v \in V$ that represents the number of times until iteration $n$ that the sample $(i,u,v,j)$ has been encountered. We define
\begin{align}\label{transprob}
    p'_n(j|i,u,v) = \frac{c_n[i][j][u][v]}{c_n[i][u][v]}, ~ \forall n \geq 1,
\end{align}
where $c_n[i][u][v] = \displaystyle \sum_{j=1}^{M} c_n[i][j][u][v]$. It is easy to see that (under an exploratory policy)
\begin{align}
\label{transprobconv}
    p'_n(j|i,u,v) \xrightarrow[]{} p(j|i,u,v), ~ \forall i,j,u,v,
\end{align}
as $n \xrightarrow[]{} \infty$, almost surely. 

Now, we propose our model-free ``generalised minimax Q-learning'' by modifying the Step-2 of the Algorithm \ref{alg:minimax Q-learning} as:
\begin{align}
    d_{n+1}(i,u,v) = w_n\Big(r(i,u,v)+\alpha\V [Q_n(Y_n(i,u,v))]\Big)\\ \nonumber
 \hspace*{2 cm} +(1-w_n)\V[Q_n(i)],
\end{align}
where the sequence $\{w_n,~ n \geq 1\}$ is updated as:
\begin{align}
    w_{n+1} = (1-\beta_n)w_n + \beta_n \Big(\frac{1}{1 - \alpha \displaystyle \min_{i,u,v}p'_n(i|i,u,v)}  \Big),
\end{align}
with $w_0 = 1$ and $\beta_n$ is a smaller time-scale step-size sequence satisfying:
$$\displaystyle\sum_{n=1}^{\infty} \beta_n = \infty, ~ \displaystyle\sum_{n=1}^{\infty} (\beta_n + \gamma_n)^2 < \infty, ~ \frac{\beta_n}{\gamma_n} \xrightarrow[]{} 0. $$

Before proceeding to convergence analysis, we state and prove the following lemma.
\begin{lemma}\label{qrange}
$||Q_w{\dagger}|| \leq B,~ 1 \leq w \leq w^*,$ where $B = \displaystyle \frac{(1+\alpha)R}{(1-\alpha)^2}$ and $R = \displaystyle \max_{i,u,v}|r(i,u,v)|$. 
\end{lemma}
\begin{proof}
First note that, the solution of the two-player Markov game $Q$ is bounded by:
$||Q|| \leq \displaystyle \frac{R}{1-\alpha}$. From Lemma \ref{l7}, for $1 \leq w \leq w^*$,
\begin{align*}
    |Q_w^{\dagger}(i,u,v)| &\leq |1-w||J^*(i)| + w|Q(i,u,v)| \\
                      & \leq \frac{\alpha}{(1-\alpha)^2}R + \frac{1}{(1-\alpha)^2}R \\
                      & \leq \displaystyle \frac{(1+\alpha)R}{(1-\alpha)^2}.
\end{align*}
\end{proof}
\subsection{Convergence Proof:}
We make use of two-time scale stochastic approximation \cite{borkar2009stochastic} to show the convergence of our algorithm. We first write the two update equations as follows:
\begin{align}
\label{ttup1}
    Q_{n+1}(i,u,v) = \Gamma_{C} \Big\{ Q_n(i,u,v) + \gamma_n (&h(Q_n,w_n)+ M_{n+1})\Big\}, \nonumber \\ & ~ \forall i,u,v
\end{align}
\begin{align}
\label{ttup2}
    w_{n+1} = w_n + \beta_n (g(w_n) + \epsilon_n),
\end{align}
where $\Gamma_{C}(P)$ is the projection of $P$ on to a set $C = [-B,B]^{S|\times |U| \times |V|}$. As the set $C$ is convex and compact, projection exists and is unique. The function $h$ is defined as: 
\begin{align*} 
h(Q_n,w_n)(i,u,v) &= H_{w_n}(Q_n)(i,u,v) - Q_n(i,u,v) \\ &= \E\Big[w_n\Big(r(i,u,v)+\alpha\V [Q_n(j)]\Big)\\& 
+(1-w_n)\V[Q_n(i)] - Q_n(i,u,v)\Big].
\end{align*}
The sequence $\{M_n\}$ defined as:
\begin{align}\label{mtdiffseq}
    M_{n+1} = w_n\Big(r(i,u,v)+\alpha\V [Q_n(Y_n(i,u,v))]\Big)\\ \nonumber
+(1-w_n)\V[Q_n(i)] - Q_n(i,u,v) - h(Q_n,w_n),
\end{align}
is a Martingale noise sequence with respect to the increasing $\sigma-$fields 
\begin{align*}
    \F_n := \{Q_0,w_0,M_0,\ldots,w_n,M_n\}, ~ n \geq 0,
\end{align*}
satisfying
\begin{align*}
    \E[||M_{n+1}||^2|\F_n] &\leq 3w_n^2\Big(\displaystyle \max_{i,u,v}|r(i,u,v)| \Big)^2 + \frac{6\alpha^2}{(1-\alpha)^2}||Q_n||^2 \\ 
                            &\leq K \big(1+||w_n||^2+||Q_n||^2\big),
\end{align*}
where $K = \max \Big\{3\Big(\displaystyle \max_{i,u,v}|r(i,u,v)| \Big)^2,\frac{6\alpha^2}{(1-\alpha)^2} \Big\}$.
The function $g$ is defined as:
\begin{align*}
    g(w_n) = \displaystyle \frac{1}{1 - \alpha \displaystyle \min_{i,u,v}p(j|i,u,v)} - w_n
\end{align*}
Finally, $\epsilon_n$ is defined as:
\begin{align*}
    \epsilon_n = \frac{1}{1 - \alpha \displaystyle \min_{i,u,v}p'_n(j|i,u,v)} - \frac{1}{1 - \alpha \displaystyle \min_{i,u,v}p(j|i,u,v)},
\end{align*}
where $p'_n$ is updated as shown in the equation \eqref{transprob}. Note that, from equation \eqref{transprobconv}, we get $\epsilon_n \xrightarrow[]{} 0$ as $n \xrightarrow[]{} 0$, almost surely. 

The updates \eqref{ttup1} and \eqref{ttup2} are of the form of two-time scale stochastic approximation updates defined in \cite{borkar2009stochastic}. To show the convergence of these updates, we prove the conditions specified in \cite{borkar2009stochastic}, below.

Before proving the conditions, we make an assumption on $\{w_n\}$ iterates. 
\begin{assumption}\label{assump1}
$w_n \leq w^*,~ \forall n \geq 1$.
\end{assumption}
We know that $w_n \in \Big[1,\displaystyle \frac{1}{1-\alpha}\Big], ~ \forall n \geq 0$. However, to prove the following lemmas, we need $w_n \leq w^* \leq \displaystyle \frac{1}{1-\alpha}$. This assumption can be satisfied by maintaining:
\begin{itemize}
    \item Very small step-size sequence $\{\beta_n\}$ in \eqref{ttup2}.
    \item Periodic update of $w_n$, i.e., $w_n$ is updated after every $T > 1$ iterations. 
\end{itemize}
Moreover, note that the $\{w_n\}$ iterates do not depend on $\{Q_n\}$ iterates.
%*********************************************************************************
% \begin{assumption}\label{assump2}
% $||Q_n|| \leq \displaystyle B, ~ \text{where} ~ \frac{R(1+\alpha)}{(1-\alpha)^2} \leq B < \infty, ~ R = \displaystyle \max_{i,u,v}|r(i,u,v)|, ~ \forall n \geq 0$, almost surely.
% \end{assumption}
% First note that, the solution of the two-player Markov game $Q$ is bounded by:
% $||Q|| \leq \displaystyle \frac{R}{1-\alpha}$. For any fixed $w \leq w^*$, the $\{Q_n\}$ iterates converge to $Q_w^{\dagger}$ almost surely. This implies that these iterates are bounded almost surely. Therefore, we can project the iterates $\{Q_n\}$ of \eqref{ttup1} to a convex and compact set $[-B,B]^{S|\times |U| \times |V|}$, provided that the solution lies in the set. To ensure that, we observe from Lemma \ref{l7} that, $\forall w$:
% \begin{align*}
%     ||Q_w^{\dagger}|| &\leq |1-w||J^*(i)| + w|Q(i,u,v)| \\
%                       & \leq \frac{\alpha}{(1-\alpha)^2}R + \frac{1}{(1-\alpha)^2}R \\
%                       & \leq \displaystyle \frac{(1+\alpha)R}{(1-\alpha)^2}.
% \end{align*}
% Therefore we can project the $\{Q_n\}$ iterates on to the set $\Bigg[\displaystyle \frac{-R}{1-\alpha}, \displaystyle \frac{R}{1-\alpha}\Bigg]^{|S|\times |U| \times |V|}$. As this set is compact and convex, the projection is well defined. 

%**********************************************************************************

%********Stability Lemma*****************************
% \begin{lemma}
% $\{Q_n, ~ n \geq 0\}$ iterates are stable almost surely.
% \end{lemma}
% \begin{proof}
% We show the stability of $\{Q_n\}$ iterates by considering the stochastic recursive inclusion:
% \begin{align}\label{sri}
%     Q_{n+1} = Q_n + \gamma_n[y_n + M_{n+1}], ~ \forall n \geq 0,
% \end{align}
% $y_n \in f(Q_n)$ where $f:\R^{|S|\times |U| \times |V|} \xrightarrow[]{} \{\text{subsets of} ~ \R^{|S|\times |U| \times |V|} \} $ is a set-valued function given by 
% \begin{align}\label{svf}
% f(Q_n) = \{H_w(Q_n) - Q_n | 1 \leq w \leq w^* \}.    
% \end{align}
% Note that the set of iterates $\{Q_n\}$ obtained using \eqref{ttup1} is subset of iterates obtained by following \eqref{sri}. Therefore, if we show the stability of iterates in \eqref{sri}, then the stability of iterates in \eqref{ttup1} is implied. To this end, we show the stability of iterates in \eqref{sri} by proving the following conditions specified for stability in \cite{ramaswamy2017generalization}.
% \begin{enumerate}
%     \item $f$ is a Marchaud map \cite{borkar2009stochastic}, i.e.,
%     \begin{itemize}
%         \item For each $Q$, $f(Q)$ given by \eqref{svf} is convex and compact.
%         \item For a given $Q$, consider $y \in f(Q)$. Then, $y$ is of form $H_w(Q) - Q$, for some $1 \leq w \leq w^*$. Then,   
%         \begin{align*}
%             ||y|| &= || H_w(Q) - Q|| \\
%                   & \leq w^*\max_{i,u,v}|r(i,u,v)| + 2 ||Q|| \\
%                   & \leq K(1+||Q||),
%         \end{align*}
% where $K = \max\{w^* \displaystyle \max_{i,u,v}|r(i,u,v)|,2\}$.
%       Therefore, 
%       \begin{align*}
%           \sup_{y \in f(Q)} ||y|| \leq K(1 + ||Q||).
%       \end{align*}
%         \item For a given sequence $\{Q_n\}$, let $Q_n \xrightarrow[]{} Q $ and $y_n \xrightarrow[]{} y$, where $y_n \in f(Q_n)$. Here $y_n$ is of form $H_{w_n}(Q_n) - Q_n$, for some $1 \leq w_n \leq w^*$. Then, 
%         \begin{align}
%             y = H_w(Q) - Q ~ \in f(Q),
%         \end{align}
% for some $1 \leq w \leq w^*$.
%     \end{itemize}
    
% \item $\{\gamma_n\}$ satisfies $\displaystyle\sum_{n=1}^{\infty} \gamma_n = \infty, ~ \displaystyle\sum_{n=1}^{\infty}\gamma_n^2 < \infty$.
% \item $\{M_n\}$ is a Martingale difference sequence as defined in \eqref{mtdiffseq} satisfies: 
% \begin{align*}
%     \E[||M_{n+1}||^2|\F_n] \leq K (1 + ||Q_n||^2), ~ n \geq 0,
% \end{align*}
% for some constant $K > 0$ and filtration $\F_n = \sigma\{Q_0,M_1,\ldots,M_n \}$.
% \item For $c \geq 1$, define $f_c(Q) = \{y ~|~ cy \in f(cQ)\}$. Further, define $f_{\infty}(Q) := \displaystyle \liminf_{c \xrightarrow[]{} \infty} f_c(x)$. For our function $f$,
% \begin{align*}
%     f_{\infty} = \{ \displaystyle \Tilde{H}_w(Q) -Q ~|~ 1 \leq w \leq w^* \},
% \end{align*}
% where 
% \begin{align*}
%     \Tilde{H}_w(Q)(i,u,v) =& \E\Big[w\Big(\alpha\V [Q(j)]\Big) \\& 
% +(1-w)\V[Q(i)]\Big],
% \end{align*}
% which corresponds to the modified Q-Bellman operator for the Markov game with single-stage rewards as zero in all states and actions of agents. Hence, $\dot Q(t) = \Tilde{H}_w(Q) -Q$ for a fixed $1 \leq w \leq w^*$, has $\{0\}$ as its globally asymptotic stable equilibrium point. Therefore, the differential inclusion $\dot Q(t) \in f_{\infty}(Q(t))$ has an attracting set $S$ with $\{0\} \subset S$. 
% \item Let $c_n \geq 1$ be an increasing sequence of integers such that $c_n \uparrow \infty$. Let $Q_n \xrightarrow[]{} Q$ and $y_n \xrightarrow[]{} y$, where $y_n \in f_{c_n}(Q_n), ~ \forall n$. Here, $y_n$ will be of form:
% \begin{align*}
%     y_n = \frac{H_{w_n}(c_nQ_n)}{c_n} - Q_n.
% \end{align*}
% Now,
% \begin{align*}
%   \displaystyle \lim_{n \xrightarrow[]{} \infty} y_n = \Tilde{H}_w(Q) - Q ~ \in f_{\infty}(Q).
% \end{align*}
% \end{enumerate}
% Under (1)-(5), generalisation of Borkar-Meyn theorem for stochastic recursive inclusions (Theorem 1 of \cite{ramaswamy2017generalization}) implies that $\{Q_n\}$ given by \eqref{sri} satisfies: 
% \begin{align*}
%     \sup_n||Q_n|| \leq \infty, ~ \text{almost surely}.
% \end{align*}
% \end{proof}
%*************End of Stability*********************
\begin{lemma}
Functions $h(Q,w)$ and $g(w)$ are Lipschitz.
\end{lemma}
\begin{proof}
Consider $p,q \in [-B,B]^{S|\times |U| \times |V|}$ and $w_1,w_2 \in [1,w^*]$. Let $R = \displaystyle \max_{i,u,v}|r(i,u,v)|$. Then,
\begin{align}
    ||h(p,w_1) - h(q,w_2)|| \leq & ||h(p,w_1) - h(q,w_1)|| +  \\ &||h(q,w_1) - h(q,w_2)||. \nonumber 
\end{align}
\begin{align*}
    ||h(p,w_1) - h(q,w_1)|| &\leq  ||H_{w_1}(p) - H_{w_1}(q)|| + ||p-q|| \\ & \leq (1-w_1+w_1\alpha)||p-q|| + ||p-q|| \\ & \leq 2||p-q||,
\end{align*}
\begin{align*}
    |(h(q,w_1) - h(q,w_2))(i,u,v)| &\leq |w_1 - w_2| \E[|r(i,u,v) \\ &+ \alpha \V[q(j)] - \V[q(i)|]
    \\ & \leq |w_1 - w_2|(R + 2B)
\end{align*}
Hence, 
\begin{align*}
    ||h(q,w_1) - h(q,w_2)|| \leq L_2 |w_1 -w_2|,
\end{align*}
where $L_2 = R + 2B$. 
Finally, 
\begin{align*}
    |g(w_1) - g(w_2)| \leq |w_1 - w_2|.
\end{align*}
Therefore the functions $h(Q,w)$ and $g(w)$ are Lipschitz. 
\end{proof}
Under fairly general conditions specified in  \cite[pages~190-191]{kushner2012stochastic}, the iterates $\{Q_n\}$ in \eqref{ttup1} track the ODE (\cite[Theorem 5.3.1]{kushner2012stochastic}):
\begin{align*}
    \dot Q(t) = \hat\Gamma (h(Q(t),w(t)),
\end{align*}
where the operator $\hat\Gamma (.)$ is defined as:
\begin{align}
    \hat\Gamma (h(Q,w)) = \displaystyle \lim_{0 <\Delta \xrightarrow[]{} 0}\frac{[\Gamma_{C}(Q+\Delta h(Q,w)) - Q]}{\Delta}.
\end{align}
Note that when $Q \in Int(C)$ (Interior of set $C$), $\hat\Gamma (h(Q,w)) = h(Q,w)$.
\begin{lemma}
\label{twol1}
$\dot Q(t) = \hat\Gamma (h(Q(t),w))$ has a globally asymptotic stable equilibrium $\lambda(w)$, where $\lambda$ is a a Lipschitz map 
\end{lemma}
\begin{proof}
For all $w\leq w^*$ (Assumption \ref{assump1}), function $h(Q(t),w)$ is a contraction (from Lemma \ref{l5}) and its fixed point lies in the set $C$ (from Lemma \ref{qrange}). In general, because of the projection of $\{Q_n\}$ iterates, the globally asymptotic stable equilibrium set of $\dot Q(t) = \hat\Gamma (h(Q(t),w))$  contains not only the fixed point of $h(Q(t),w)$, but also the boundary points of the set $C$. However, we have already proved in Theorem \ref{thm1} that for a fixed $w$, the standard $\{Q_n\}$ iterates (without projection) converge to the fixed point of $h(Q(t),w)$. Therefore, the projected iterates in \eqref{ttup1} also converge to the fixed point $Q^{\dagger}_{w}$. 
Now, consider two relaxation parameters $w_1 \leq w^*$ and $w_2 \leq w^*$. Then,
\begin{align}
    &|\lambda(w_1) - \lambda(w_2)| = ||Q^{\dagger}_{w_1} - Q^{\dagger}_{w_2}||.
\end{align}
Now,
\begin{align}
    &|(Q^{\dagger}_{w_1} - Q^{\dagger}_{w_2})(i,u,v)| \nonumber \\  & = \Big{|}w_1\bigg{(}r(i,u,v)+\alpha \sum^{M}_{j=1}p(j|i,u,v)\V[Q^{\dagger}_{w_1}(j)]\bigg{)} \nonumber \\ & +(1-w_1) \V[Q^{\dagger}_{w_1}(i)] \nonumber \\ \nonumber &- w_2\bigg{(}r(i,u,v)+\alpha \sum^{M}_{j=1}p(j|i,u,v)\V[Q^{\dagger}_{w_2}(j)]\bigg{)} \nonumber \\ & -(1-w_2) \V[Q^{\dagger}_{w_2}(i)] \Big{|}  \label{l6step1}
    \\ & \leq  |r(i,u,v) (w_1 - w_2)| + \alpha \displaystyle \max_i |\V[Q(i)]| |w_1 - w_2| \nonumber \\ 
    &+ |\V[Q(i)] (w_1 - w_2)| \label{l6step2} \\
    & \leq |w_1 - w_2| (\displaystyle \max_{i,u,v}|r(i,u,v)| + (\alpha +1) \max_i |\V[Q(i)]|).
\end{align}
Expression \eqref{l6step2} follows from \eqref{l6step1} by Lemma \ref{l7} where we have showed that: 
\begin{align}
    \V[Q^{\dagger}_{w_1}(i)] = \V[Q^{\dagger}_{w_2}(i)] = \V[Q(i)],
\end{align}
where $Q$ is the solution of the min-max Q-Bellman equation of the game. 
Therefore, 
\begin{align}
    |\lambda(w_1) - \lambda(w_2)| \leq M|w_1 - w_2|,
\end{align}
where $M =\displaystyle \max_{i,u,v}|r(i,u,v)| + (\alpha +1) \max_i |\V[Q(i)]|$ and hence $\lambda(w)$ is Lipschitz. 
\end{proof}
%***********************************************************
% \begin{lemma}
% \label{twol2}
% $\dot w(t) = g(w(t))$ has a globally asymptotic stable equilibrium $w^*$.
% \end{lemma}
% \begin{proof}
% Let $g_\infty(w) = \displaystyle \lim_{r \xrightarrow[]{} \infty} \frac{g(rw)}{r}$. The function $g_\infty(w)$ exists and is equal to $-w$. The origin is an asymptotically stable equilibrium for the ODE
% \begin{align*}
%     \dot w = g_\infty(w),
% \end{align*}
% with $V(w) = \frac{w^2}{2}$ serving as an associated Lyapunov function. 
% Therefore function $g(w(t))$ has an isolated equilibrium point at $w$ such that:
% \begin{align}
%     w = \displaystyle \frac{1}{1 - \alpha \displaystyle \min_{i,u,v}p(j|i,u,v)}.
% \end{align}
% By definition, such a point is unique and is equal to $w^*$. 
% \end{proof}
%***********************************************************
\begin{lemma}
\label{twol2}
$\{w_n\}$ iterates gives by \eqref{ttup2} satisfy $w_n \xrightarrow[]{} w^*$ with probability 1, where
\begin{align*}
    w^*=\displaystyle\min_{i,u,v}\Bigg{\{}\frac{1}{1-\alpha p(i|i,u,v)}\Bigg{\}}.
\end{align*}
\end{lemma}
\begin{proof}
The ODE associated with $\{w_n\}$ iterates is given by:
\begin{align*}
    \dot w = g(w) = -w + w^*
\end{align*}
Let $g_\infty(w) = \displaystyle \lim_{r \xrightarrow[]{} \infty} \frac{g(rw)}{r}$. The function $g_\infty(w)$ exists and is equal to $-w$. The origin is an asymptotically stable equilibrium for the ODE
\begin{align*}
    \dot w = g_\infty(w) = -w,
\end{align*}
with $V(w) = \frac{w^2}{2}$ serving as an associated Lyapunov function. Therefore, we have \cite{borkar2009stochastic} $w_n \xrightarrow[]{} w^*$ almost surely. 
\end{proof}



% \begin{lemma}
% \label{twol3}
% $\sup_{n}(||Q_n|| + ||w_n||) < \infty$ almost surely. 
% \end{lemma}
% \begin{proof}
% For $w_n \leq w^*$ (Assumption \ref{assump1}), the sequence $\{Q_{n}\}$ is convergent and therefore bounded for all finite pairs $(i,u,v)$ almost surely. Hence, $||Q_n|| + ||w_n||$ is bounded $\forall n \geq 1$ almost surely. 
% \end{proof}

\begin{theorem}
$(Q_n,w_n) \xrightarrow[]{} (\lambda(w^*),w^*)$, almost surely.
\end{theorem}
\begin{proof}
The result follows from applying foregoing Lemmas to \cite[Theorem 2,~ Chapter 6]{borkar2009stochastic}. Here $\lambda(w^*) = Q^{\dagger}_{w^*}$ is the fixed point of $H_{w^*}$. 
\end{proof}
\color{black}


==> extension.tex <==
\section{Extension to general stochastic games} \label{extnsn}
\color{black}

In the previous section, we have proposed a model-free algorithm for solving the two-player zero-sum stochastic games. However, it assumes a special structure on the games, that is $w^* > 1$. This may not be true, in general. In this section, we extend our algorithm to the general stochastic games. 

It is noted in the literature \cite{kahan2002gauss} that successive relaxation technique works faster when $w$ is chosen in between $[1,2]$. However, the exact value of $w$, to achieve faster convergence, depends on the problem. Moreover, the only fact known about general two-player stochastic games is that $w^* \geq 1$. The idea of our algorithm, therefore, is to construct a sequence $\{w_n\}$, with $w_0 = 2$ and $w_n \downarrow 1$. 

We now propose our model-free algorithm for general two-player stochastic games, which we refer to as ``Successive Over-relaxed minimax Q-learning''. Consider a sequence $\{u_n\}$ with $u_0 = 2$ and $u_n \xrightarrow{} 1$. For example, $u_0 = 2$ and $u_n = 1 +\frac{1}{n}, ~ n \geq 1$ satisfies the specified condition. 

The new update equations are as follows:
\begin{align}
\label{tttup1}
    Q_{n+1}(i,u,v) = Q_n(i,u,v) + \gamma_n (h(Q_n,w_n)+ M_{n+1}), ~ \forall i,u,v \\
% \end{align}
% \begin{align}
\label{tttup2}
    w_{n+1} = w_n + \gamma_n (g(w_n) + \epsilon_n),
\end{align}
where $h(Q_n,w_n)$ and $M_{n+1}$ are as defined in \eqref{ttup1}-\eqref{ttup2}, $g(w_n) = 1 - w_n$ and $\epsilon_n = u_n -1$, with $w_0 = 2$. Note that, by our definition of $\{u_n\}$, we have $\epsilon_n \xrightarrow{} 0,$ as $n \xrightarrow{} \infty$.

As before, let us write the updates in \eqref{tttup1}-\eqref{tttup2} in a combined form as:
\begin{align}\label{combiternew}
    x_{n+1} = \Gamma_{C}\Big{(} x_n + \gamma_n(f(x_n)+M'_{n+1}+ \epsilon'_n) \Big{)},
\end{align}
where $x_n =
\begin{pmatrix}
Q_n \\
w_n 
\end{pmatrix}$, $f(x_n) =
\begin{pmatrix}
H_{w_n}(Q_n) - Q_n \\
1 - w_n
\end{pmatrix}$, $M'_{n+1} = \begin{pmatrix}
M_{n+1} \\
0
\end{pmatrix}$, $\epsilon'_n = \begin{pmatrix}
0 \\
\epsilon_n
\end{pmatrix}$, and $\Gamma_{C}$ is the projection operator that projects the iterates in to the set $C$.

It is clear from \cite[Chapter 5.4]{borkar2009stochastic} that the iterates $\{x_n\}$ track the ODE given by:
\begin{align}\label{proj-ext}
    \dot x = \hat \Gamma_{x(t)}\Big(f(x(t) \Big),
\end{align}
where the operator $\hat \Gamma_{x}(y) = \displaystyle \lim_{\delta \downarrow 0} \frac{\Gamma_{C}(x+\delta y) - \Gamma_{C}(x)}{\delta}$. 

We assume that the set $C$ is large enough to contain $Q^{\dagger}$. Note that, we do not use the projection in experiments. It is done in the analysis to ensure the stability of iterates. 

It is clear from our earlier analysis that $x^* = \begin{pmatrix}
Q^{\dagger} \\
1
\end{pmatrix}$ is the unique equilibrium point inside the set $C$. Along with this $x^*$, there can be other spurious equilibrium points on the boundary of the set $C$ for the ODE \eqref{proj-ext} (due to the projection). However, if the $\{w_n\}$ iterates are well controlled, the driving field for the $\{Q_n\}$ iterates will be towards the inside of the set $C$ and hence,
\begin{align}
    Q_{n} \xrightarrow[]{} Q^{\dagger}, ~ \text{almost surely}.
\end{align}
\color{black}
